GraphSnapShot: Caching Local Structure for Fast Graph Learning

In our recent research, we have developed a framework called GraphSnapShot, which has been proven an useful tool for graph learning acceleration. GraphSnapShot is a framework for fast cache, storage, retrieval and computation for graph learning. It can quickly store and update the local topology of graph structure and allows us to track patterns in the structure of graph networks, just like take snapshots of the graphs. In experiments, GraphSnapShot shows efficiency, it can achieve up to 30% training acceleration and 73% memory reduction for lossless graph ML training compared to current baselines such as dgl.This technique is particular useful for large dynamic graph learning tasks such as social media analysis and recommendation systems to process complex relationships between entities. The code for GraphSnapShot is publicly available at https://github.com/NoakLiu/GraphSnapShot.

==> content/archi.tex <==
\section{GraphSnapShot Architecture}

GraphSnapShot is designed to solve the inefficacy for current graph masking methods on large graphs. Typical distributed graph processing System such as Marius \citep{DBLP:journals/corr/abs-2101-08358}, will re-sample all the local structure each time, and load corresponding node embeddings from disk, which is time-consuming. GraphSnapShot proposing a new method for quick local structure retrieval by integrating the benefits of both static and dynamic processing. In the preprocessing phase, a static graph snapshot is sampled and stored in memory from the disk. Then, in the computation phase, the algorithm re-samples the graph snapshot, using a mix of data partially from memory and partially from disk. Concurrently, a smaller, dynamic snapshot is sampled from the disk. This dynamic snapshot is crucial as it is used to swap with the portion of the graph stored in memory. This process ensures the computation can always learn "fresh" snapshot without overwhelming the memory capacity. GraphSnapShot allows the algorithm to continuously update and adapt to changes in the graph while maintaining a manageable memory footprint, making it an effective tool for processing large, dynamic graph data.


\begin{algorithm}[h]
\caption{GraphSnapShot Process}
\begin{algorithmic}[2]

\Function{Process}{$G$, $\alpha$, $N$}
    \State $sG \gets$ \Call{Preprocess}{$G$}
    \While{($In Computation$)}
        \State $dNodes \gets$ \Call{DynamicSample}{$G$, $\alpha$, $N$}
        \State $rNodes \gets$ \Call{ReSample}{$sG$, $(1 - \alpha)$, $N$}
        \State $uG \gets$ \Call{Combine}{$dNodes$, $rNodes$}
        \State $sG \gets$ \Call{Remove}{$sG$, $rNodes$}
        \State $sG \gets$ \Call{Add}{$sG$, $dNodes$}
        \State $result \gets$ \Call{Compute}{$uG$}
    \EndWhile
    \State \Return $result$
\EndFunction

\end{algorithmic}
\end{algorithm}

\begin{algorithm}[h]
\caption{Static Sampling and Dynamic ReSampling}
\begin{algorithmic}[1]

\Function{Preprocess}{$G$}
    \State $sG \gets$ \Call{StaticSample}{$G$}
    \State \Return $sG$
\EndFunction

\Function{DynamicSample}{$G$, $\alpha$, $N$}
    \State $num \gets \alpha \times N$
    \State $sNodes \gets$ \Call{SampleFromDisk}{$G$, $num$}
    \State \Return $sNodes$
\EndFunction

\Function{ReSample}{$sG$, $\alpha$, $N$}
    \State $num \gets \alpha \times N$
    \State $sNodes \gets$ \Call{SampleFromMemory}{$sG$, $num$}
    \State \Return $sNodes$
\EndFunction
\end{algorithmic}
\end{algorithm}

\begin{algorithm}[h]
\caption{Local Snapshot Swap}
\begin{algorithmic}[2]

\Function{Add}{$G$, $Nodes$}
    \State $G \gets G \cup Nodes$
    \State $Nodes \gets$ \Call{MoveToMemoryFromDisk}{$Nodes$}
    \State \Return $G$
\EndFunction

\Function{Remove}{$G$, $Nodes$}
    \State $G \gets G - Nodes$
    \State $Nodes \gets$ \Call{MoveToDiskFromMemory}{$Nodes$}
    \State \Return $G$
\EndFunction

\end{algorithmic}
\end{algorithm}

\begin{figure}[h]
\centering
\includegraphics[width=1\linewidth]{SSDReS.png}
\caption{GraphSnapShot Model, code: \href{https://github.com/NoakLiu/GraphSnapShot}{https://github.com/NoakLiu/GraphSnapShot}} %\footnotemark
\end{figure}

% \footnotetext{GraphSnapShot Code: \url{https://github.com/NoakLiu/GraphSnapShot}.}

\begin{figure}[h]
\centering
\includegraphics[width=1\linewidth]{figures/Disk_Cache_Memory_GraphSnapShot.png}
\caption{Disk-Cache-CPU/GPU Architecture for GraphSnapShot}
\end{figure}

In the GraphSnapShot system, disks are used to store edge and node embedding information, while computational resources (CPU/GPU) are utilized for neural network computations (such as backpropagation) and local structure masking. Additionally, the cache is employed to store the K-V pairs information of the sampled structure.

% \begin{itemize}
%     \item Disk: Store node embeddings informaiton.
%     \item Cache: Store frequent K-V pair of GraphSnapShot to accelerate graph learning.
%     \item CPU/GPU: Computational Resources to compute the graph local structure and resample the graph local structure.
% \end{itemize}

\begin{itemize}
    \item Disk: Persistent storage of graph structure information, such as edges and node embedding parameters. Those embeddings are stored long-term and loaded into memory when needed for further processing and analysis.
    \item Cache: Store frequent K-V pairs of GraphSnapShot to accelerate graph learning. These K-V pairs include the identifiers of the sampled structure nodes and their embedding parameters, allowing for more efficient repeated access to the graph data.
    \item CPU/GPU: Computational Resources to responsible for performing local structure computations on the graph, including neural network forward and backward propagation as well as the dynamic resampling and masking of the graph's local structure.
\end{itemize}

==> content/archi_n.tex <==
\section{GraphSnapShot Architecture}

GraphSnapShot is designed to overcome the inefficiencies of current graph masking and sampling methods, particularly for large and dynamic graphs. Traditional distributed graph processing systems, such as Marius \citep{DBLP:journals/corr/abs-2101-08358}, repeatedly re-sample entire local structures and load corresponding node embeddings from disk for each computation step. This approach is not only time-consuming but also memory-intensive. GraphSnapShot introduces a hybrid caching mechanism that combines \textbf{static caching} and \textbf{dynamic updates}, enabling efficient retrieval of local structures while reducing redundant computation.

\subsection{System Components}

The GraphSnapShot framework integrates three key components: disk, cache, and computational resources (CPU/GPU). Each component plays a specific role in enabling efficient graph learning:

\begin{itemize}
    \item \textbf{Disk}: Persistent storage for graph structure information, including edges and node embedding parameters. These embeddings are stored long-term and loaded into memory only when needed for further processing or updates.
    \item \textbf{Cache}: Temporary storage for frequently accessed key-value (K-V) pairs. These pairs include identifiers of sampled subgraph nodes and their embeddings, allowing repeated access to the most relevant data without additional disk I/O operations.
    \item \textbf{CPU/GPU}: Handles neural network computations, such as forward and backward propagation, as well as dynamic resampling and masking of local graph structures. These resources efficiently process the cached data and interact with the disk for updates.
\end{itemize}

Each component contributes to the overall system's efficiency. The cache bridges the latency gap between the disk and computation, while the CPU/GPU ensures fast processing of cached graph data.

\subsection{Hybrid Caching Mechanism}

GraphSnapShot maintains a cached representation of the graph that balances static and dynamic components. Let \( G = (V, E) \) denote the graph, where \( V \) is the set of nodes and \( E \) is the set of edges. At any timestep \( t \), the cached snapshot \( G_{\text{snapshot}, t} \) is expressed as:
$$
G_{\text{snapshot}, t} = \alpha G_{\text{static}} + (1 - \alpha) G_{\text{dynamic}, t},
$$
where:
\begin{itemize}
    \item \( G_{\text{static}} \) is a static snapshot, precomputed during the preprocessing phase.
    \item \( G_{\text{dynamic}, t} \) captures updates to the graph's structure at time \( t \).
    \item \( \alpha \in [0, 1] \) is a parameter controlling the weight of static and dynamic components.
\end{itemize}

\paragraph{Static Sampling.}  
In the preprocessing phase, a static snapshot \( G_{\text{static}} \) is created by sampling $k$-hop neighborhoods around a subset of nodes \( V_s \subset V \). Formally:
$$
G_{\text{static}} = \bigcup_{v \in V_s} \mathcal{N}_k(v),
$$
where \( \mathcal{N}_k(v) \) represents the $k$-hop neighborhood of node \( v \). This snapshot is stored in memory for fast access during computation.

\paragraph{Dynamic Resampling.}  
During computation, GraphSnapShot updates the cache with a dynamic snapshot \( G_{\text{dynamic}, t} \), sampled from the disk. Let \( V_d \subset V \) denote the set of nodes selected for dynamic updates. The dynamic snapshot is defined as:
$$
G_{\text{dynamic}, t} = \bigcup_{v \in V_d} \mathcal{N}_k(v).
$$

The cached snapshot \( G_{\text{snapshot}, t+1} \) is updated as:
$$
C_{t+1} = \gamma G_{\text{dynamic}, t} + (1 - \gamma) C_t,
$$
where \( \gamma \) is the refresh rate.

This hybrid caching mechanism ensures that frequently accessed structures are stored in memory while capturing the latest graph updates dynamically.

\subsection{Advantages of Hybrid Caching}

The hybrid caching mechanism provides several key benefits:
\begin{enumerate}
    \item \textbf{Reduced Latency:} Static snapshots minimize the need for repeated disk access, reducing latency during computation.
    \item \textbf{Dynamic Adaptation:} The dynamic component ensures that the cache reflects recent changes in graph topology, improving accuracy.
    \item \textbf{Memory Efficiency:} By combining static and dynamic components, the cache uses memory resources optimally.
\end{enumerate}

\subsection{GraphSnapShot Workflow}

The complete workflow alternates between static sampling, dynamic resampling, and cache updates. The process is summarized in Algorithm~\ref{alg:GraphSnapShotWorkflow}.

\begin{algorithm}[h]
\caption{GraphSnapShot Workflow}
\label{alg:GraphSnapShotWorkflow}
\begin{algorithmic}[1]
\Function{GraphSnapShot}{$G, \alpha, N$}
    \State $C \gets$ \Call{StaticSample}{$G$} \Comment{Precompute static snapshot}
    \While{Computation Continues}
        \State $G_{\text{dynamic}} \gets$ \Call{DynamicSample}{$G, \alpha, N$}
        \State $G_{\text{resample}} \gets$ \Call{ReSample}{$C, (1 - \alpha), N$}
        \State $G_{\text{update}} \gets$ \Call{Combine}{$G_{\text{dynamic}}, G_{\text{resample}}$}
        \State $C \gets$ \Call{UpdateCache}{$C, G_{\text{dynamic}}, G_{\text{resample}}$}
        \State $result \gets$ \Call{Compute}{$G_{\text{update}}$}
    \EndWhile
    \State \Return $result$
\EndFunction
\end{algorithmic}
\end{algorithm}

\subsection{System Integration}

The GraphSnapShot framework integrates seamlessly with modern computational resources. Its architecture is designed to leverage disk, cache, and CPU/GPU components efficiently. Figure~\ref{fig:GraphSnapShotArchitecture} illustrates this integration.

\begin{figure}[h]
\centering
\includegraphics[width=1\linewidth]{figures/Disk_Cache_Memory_GraphSnapShot.png}
\caption{System Architecture of GraphSnapShot. The architecture integrates disk for persistent storage, cache for frequently accessed structures, and CPU/GPU for efficient computation.}
\label{fig:GraphSnapShotArchitecture}
\end{figure}

\subsection{Performance Impact}

GraphSnapShot significantly accelerates graph learning by:
\begin{enumerate}
    \item \textbf{Eliminating Redundant Computation:} Cached snapshots reduce the need for repeated sampling and recomputation.
    \item \textbf{Optimizing Memory Usage:} By combining static and dynamic caching, the system balances memory efficiency and computational needs.
    \item \textbf{Enhancing Scalability:} The hybrid design allows efficient handling of large-scale and dynamic graphs, supporting real-world applications.
\end{enumerate}

\section{Conclusion}

GraphSnapShot introduces a novel approach to graph learning by integrating static and dynamic caching mechanisms. Its ability to dynamically adapt to graph changes while maintaining efficient memory usage makes it a powerful tool for large-scale graph processing. Future work will explore its application to heterogeneous graphs and distributed systems, extending its scalability further.


==> content/archi_nn.tex <==
\section{GraphSnapShot Architecture}

GraphSnapShot addresses the inefficiencies of traditional graph masking and sampling methods in handling large-scale, dynamic graphs. Systems such as Marius \citep{DBLP:journals/corr/abs-2101-08358} rely on repeated resampling of local structures and loading embeddings from disk, incurring significant computational and memory overhead. GraphSnapShot introduces a hybrid caching mechanism that integrates \textbf{static caching} and \textbf{dynamic resampling}, enabling efficient graph learning while minimizing redundant operations.

\subsection{System Components}

The GraphSnapShot framework consists of three main components: \textbf{disk}, \textbf{cache}, and \textbf{CPU/GPU}. Each plays a specific role in managing the graph data flow:

\begin{itemize}
    \item \textbf{Disk}: Stores the complete graph structure \( G = (V, E) \), including edges, node embeddings \( \mathbf{H}_v \in \mathbb{R}^{d} \), and metadata. These are persistently stored and loaded into memory only when required for computation.
    \item \textbf{Cache}: Maintains frequently accessed subgraphs and their embeddings. Cached subgraphs \( G_{\text{cached}, t} \subset G \) are represented as key-value (K-V) pairs, where keys are node identifiers and values are corresponding embeddings \( \mathbf{H}_v \).
    \item \textbf{CPU/GPU}: Handles neural network computations such as forward and backward passes, as well as dynamic resampling and masking operations for local graph structures.
\end{itemize}

These components form a hierarchical architecture where the cache bridges the latency gap between disk and computational resources, while the CPU/GPU ensures efficient processing.

\subsection{Hybrid Caching Mechanism}

The core of GraphSnapShot is a hybrid caching mechanism that combines static and dynamic components. Let \( G = (V, E) \) represent the graph. At any time \( t \), the cached snapshot \( G_{\text{snapshot}, t} \) is expressed as:
$$
G_{\text{snapshot}, t} = \alpha G_{\text{static}} + (1 - \alpha) G_{\text{dynamic}, t},
$$
where:
\begin{itemize}
    \item \( G_{\text{static}} \): A static snapshot computed during preprocessing.
    \item \( G_{\text{dynamic}, t} \): A dynamic snapshot updated during computation.
    \item \( \alpha \): A parameter controlling the relative contributions of static and dynamic components, with \( \alpha \in [0, 1] \).
\end{itemize}

\paragraph{Static Sampling.}  
The static snapshot \( G_{\text{static}} \) captures $k$-hop neighborhoods around a subset of nodes \( V_s \subset V \), defined as:
$$
G_{\text{static}} = \bigcup_{v \in V_s} \mathcal{N}_k(v),
$$
where \( \mathcal{N}_k(v) \) represents the $k$-hop neighborhood of node \( v \). Static sampling reduces disk I/O by precomputing and caching frequently accessed graph regions.

\paragraph{Dynamic Resampling.}  
During computation, dynamic resampling updates the cache with changes in graph topology. Let \( V_d \subset V \) denote the set of nodes selected for updates. The dynamic snapshot is given by:
$$
G_{\text{dynamic}, t} = \bigcup_{v \in V_d} \mathcal{N}_k(v).
$$
The updated cache at time \( t+1 \) is expressed as:
$$
C_{t+1} = \gamma G_{\text{dynamic}, t} + (1 - \gamma) C_t,
$$
where \( \gamma \) controls the refresh rate.

\subsection{Hierarchical Cache Design}

To further optimize memory and computation, GraphSnapShot employs a hierarchical cache structure. Let \( C_t^{(i)} \) denote the cached snapshot at level \( i \). The update rule for a multi-level cache is defined as:
$$
C_t^{(i)} = 
\begin{cases}
\alpha^{(i)} G_{\text{dynamic}, t} + (1 - \alpha^{(i)}) C_{t-1}^{(i)}, & \text{if } i = 1, \\
\beta^{(i)} C_t^{(i-1)} + (1 - \beta^{(i)}) C_{t-1}^{(i)}, & \text{if } i > 1,
\end{cases}
$$
where \( \alpha^{(i)} \) and \( \beta^{(i)} \) control the contributions of the dynamic snapshot and the previous cache level.

\subsection{Dynamic Sampling Optimization}

Dynamic resampling balances computational cost and cache quality. The optimization objective is:
$$
\min_{G_{\text{dynamic}, t}} \mathcal{C}(G_{\text{dynamic}, t}) - \lambda \mathcal{Q}(G_{\text{dynamic}, t}),
$$
where:
$$
\mathcal{C}(G_{\text{dynamic}, t}) = \sum_{v \in V_d} \|\mathcal{N}_k(v)\|, \quad 
\mathcal{Q}(G_{\text{dynamic}, t}) = \sum_{v \in V_d} \|\nabla_{\mathcal{L}}(\mathcal{N}_k(v))\|,
$$
and \( \lambda \) balances computation cost \( \mathcal{C} \) and cache quality \( \mathcal{Q} \).

\subsection{GraphSnapShot Workflow}

The complete GraphSnapShot process is summarized in Algorithm~\ref{alg:GraphSnapShotWorkflow}.

\begin{algorithm}[h]
\caption{GraphSnapShot Workflow}
\label{alg:GraphSnapShotWorkflow}
\begin{algorithmic}[1]
\Function{GraphSnapShot}{$G, \alpha, N$}
    \State $C \gets$ \Call{StaticSample}{$G$} \Comment{Precompute static snapshot}
    \While{Computation Continues}
        \State $G_{\text{dynamic}} \gets$ \Call{DynamicSample}{$G, \alpha, N$}
        \State $G_{\text{resample}} \gets$ \Call{ReSample}{$C, (1 - \alpha), N$}
        \State $G_{\text{update}} \gets$ \Call{Combine}{$G_{\text{dynamic}}, G_{\text{resample}}$}
        \State $C \gets$ \Call{UpdateCache}{$C, G_{\text{dynamic}}, G_{\text{resample}}$}
        \State $result \gets$ \Call{Compute}{$G_{\text{update}}$}
    \EndWhile
    \State \Return $result$
\EndFunction
\end{algorithmic}
\end{algorithm}

\subsection{Performance Advantages}

GraphSnapShot accelerates graph learning through:
\begin{enumerate}
    \item \textbf{Reduced Latency:} Precomputed static snapshots minimize disk I/O.
    \item \textbf{Dynamic Adaptation:} Resampling ensures the cache reflects graph updates.
    \item \textbf{Memory Efficiency:} Hierarchical caching optimally balances memory and computation.
    \item \textbf{Scalability:} The hybrid design supports large and dynamic graphs.
\end{enumerate}


==> content/background.tex <==
\section{Background}

Local structure analysis in graph learning applications are fundamental for understanding and analyzing complex networks in various domains. This concept pertains to the idea of capturing the localized patterns and relationships within a large graph structure. Efficient graph structure learning are crucial in various applications, from social network analysis to bioinformatics, where useful hidden pattern are discovered by graph structure learning. %as they allow for the  study of individual nodes and their direct connections within the network.

The GraphSnapShot framework we proposed provide insight to study graph learning by using dynamically updated local graph snapshots. GraphSnapShot is particularly valuable in large-scale networks where global analysis can be computationally intensive and less informative for certain types of inquiries. By focusing on local structures, researchers can detect community patterns, identify influential nodes, and understand local clustering behaviors in a more efficient way.

Applications of local structure learning are diverse and impact several fields:

\begin{itemize}
  \item \textbf{Social Network Analysis:} Understanding individual or entity interactions within a network to reveal social dynamics and community formation.
  \item \textbf{Bioinformatics:} In biological networks, local structures assist in identifying functional modules or predicting protein interactions.
  \item \textbf{Recommendation Systems:} Improving recommendation accuracy by focusing on immediate user-item interaction patterns.
  \item \textbf{Network Security:} Analyzing local patterns for detecting anomalies or potential security breaches.
\end{itemize}

==> content/conclusion.tex <==
% \begin{figure}[H]
% \centering
% \includegraphics[width=1\linewidth]{SSDReS.png}
% \caption{GraphSnapShot Model}
% \end{figure}



\section{Empirical Analysis and Conclusion}

We use the Deep Graph Library (DGL\citep{wang2019deep}) and torch framework to implement GraphSnapShot, leveraging its efficient handling of graph data structures and operations. Our implementation involves loading the graph, applying the graph splitting based on node degree, and then processing each subgraph with the respective sampling technique. We evaluated the performance of our new models on datasets in ogbn-benchmark\citep{hu2020open}. The results show that GraphSnapShot can significantly reduce training time and memory usage without compromising the quality of GNN training. Emprically it beat the traditional dgl and nn samplers in speed while maintain the performance.


\subsection{Theoretial Analysis of Traditional Disk-Memory Strategy and Our Disk-Cache-Memory Strategy}

In the traditional Graph System like Marius\citep{DBLP:journals/corr/abs-2101-08358}, a disk-cache model is deployed, where the graph structure is resampled each time from the disk into the memory for computation. In our current GraphSnapShot model, we deploy a disk-cache-memory model where K-V pair for reused graph structure are stored in the cache to promote the system performance.

Theoretically, if we denote the batch processing size as $S(B)$, the cache size as $S(C)$ and the cache refreshing rate as $\alpha$, and the processing speed of cache as $v_c$, and the processing speed of memory as $v_m$. Then we can get the batch average processing time for disk-memory model as $\frac{S(G)}{v_m}$ and the batch average processing time for disk-cache-memory model as $\frac{S(B)-S(C)}{v_m}+\frac{(1-\alpha) * S(C)}{v_c}$.

% \subsection{Experimental Analysis for Different Cache Refreshing Strategies in GraphSnapShot}

% \begin{figure}[H]
%     \centering
%     \includegraphics[width=0.6\textwidth]{figures/res.png}
%     \caption{System Performance Evaluation}
%     \label{fig:enter-label}
% \end{figure}

% In our experiments, we test the performance for different methods of cache refreshing stratgies, where the cache is partially, or full updated, or cache is not used and fully rely on disk and memory inter-communication.

% In our experiments, we evaluate the performance of various cache refreshing strategies, where the cache is either partially or fully updated, or not used at all. The experimental results shows that the partially updated strategy has the best performance in  time-fast and memory efficient, while reach the similar accuracy compared to other two strategies.

% ** In our experiments, ... to do A, B and C: all vis in the appendix for different rates. (Mem, Acc, Training time)

% In our experiments, we assess the performance of different cache refreshing strategies, wherein the cache is either partially or fully updated, or not utilized at all. The experimental results show that the strategy of partially updating the cache yields the best performance in terms of speed and memory efficiency while achieving similar accuracy compared to the other two strategies.

% Give out the experimental table

% We conduct experiments on different local domain of the 

% ** add some modules for improvements on different settings.

\subsection{Training Time Reduction Analysis}
The provided table presents a detailed comparison of training time acceleration for various computational methods relative to the baseline method FBL. It quantitatively illustrates the percentage reduction in training times when employing FCR, FCR-shared cache, OTF, and OTF-shared cache methods across three distinct settings: \texttt{[20, 20, 20]}, \texttt{[10, 10, 10]}, and \texttt{[5, 5, 5]}. Each entry reflects the efficiency gains achieved by the respective method, highlighting how advancements in computational techniques can significantly decrease the time required for model training.

\begin{table}[H]
\centering
\caption{Training Time Acceleration Percentage Relative to FBL}
\label{tab:acceleration_percentage}
\begin{tabular}{|c|c|c|c|}
\hline
\textbf{Method/Setting} & \textbf{[20, 20, 20]} & \textbf{[10, 10, 10]} & \textbf{[5, 5, 5]} \\
\hline
FCR & 7.05\% & 14.48\% & 13.76\% \\
\hline
FCR-shared cache & 7.69\% & 14.33\% & 14.76\% \\
\hline
OTF & 11.07\% & 23.96\% & 23.28\% \\
\hline
OTF-shared cache & 13.49\% & 25.23\% & 29.63\% \\
\hline
\end{tabular}
\end{table}

The training time comparison table reveals that the \textbf{OTF-shared cache} method consistently provides the most substantial time accelerations, achieving up to \textbf{29.63\%} faster training times than the FBL method, particularly in the smallest setting. This performance underscores its effectiveness in scenarios demanding quick model training. The \textbf{FCR} methods, both with and without shared caching, offer steady improvements, enhancing training speeds by approximately \textbf{7\% to 14.76\%}. Notably, the \textbf{OTF} method shines in smaller settings, suggesting increased efficiency in less complex computational tasks. The positive impact of shared caching across the FCR and OTF methods indicates that optimized resource management can lead to significant reductions in training times, making these methods highly beneficial in high-performance computing environments where reducing time is essential.

\subsection{Runtime Memory reduction Analysis}

From the visualizations and data provided in the table of runtime memory reduction analysis, it is evident that the computational methods FCR, FCR-shared cache, OTF, and OTF-shared cache demonstrate significant improvements in reducing runtime memory usage compared to the baseline FBL method up to 90\%.

\begin{figure}[H]
\centering
\includegraphics[width=0.7\linewidth]{figures/runtime_mem_products.png}
\caption{Runtime Memory Reduction}
\end{figure}

\subsection{GPU Reduction Analysis}

This significant reduction in GPU memory usage demonstrates the effectiveness of the GraphSnapShot methodology. By intelligently balancing the trade-off between full storage of sparse graph regions and sampling of dense graph regions, the proposed approach greatly enhances memory efficiency, which is particularly beneficial for large-scale graph processing tasks.

\begin{table}[H]
\centering
\caption{GPU Storage Optimization Comparison}
\label{tab:storage_optimization}
\begin{tabular}{lccc}
\hline
\textbf{Dataset} & \textbf{Original} & \textbf{Optimized} & \textbf{Compression} \\ \hline
ogbn-arxiv            & 1,166,243        & 552,228           & 52.65\%              \\
ogbn-products         & 123,718,280      & 20,449,813        & 83.47\%              \\
ogbn-mag              & 5,416,271        & 556,904           & 89.72\%              \\ \hline
\end{tabular}
\end{table}

\begin{figure}[H]
\centering
% 第一个图像
\begin{minipage}[b]{0.32\textwidth}
    \includegraphics[width=\textwidth]{figures/gpu_by_thrs_mag.png}
\end{minipage}
\hfill % 添加间隙
% 第二个图像
\begin{minipage}[b]{0.32\textwidth}
    \includegraphics[width=\textwidth]{figures/gpu_by_thrs_arxiv.png}
\end{minipage}
\hfill % 添加间隙
% 第三个图像
\begin{minipage}[b]{0.32\textwidth}
    \includegraphics[width=\textwidth]{figures/gpu_by_thrs_products.png}
\end{minipage}

\caption{GPU Reduction Visualizations for Datasets (ogbn-arxiv, products and mag)}
\label{fig:gpu-reductions}
\end{figure}


% \begin{figure}[H]
% \centering
% \includegraphics[width=0.5\linewidth]{figures/gpu_by_thrs_mag.png}
% \caption{GPU Reduction Visualization for ogbn-mag}
% \end{figure}

% \begin{figure}[H]
% \centering
% \includegraphics[width=0.5\linewidth]{figures/gpu_by_thrs_arxiv.png}
% \caption{GPU Reduction Visualization for ogbn-arxiv}
% \end{figure}

% \begin{figure}[H]
% \centering
% \includegraphics[width=0.5\linewidth]{figures/gpu_by_thrs_products.png}
% \caption{GPU Reduction Visualization for ogbn-products}
% \end{figure}

\subsection{Fluent Generation Analysis}

The partial fetch and partial refresh mode are designed to achieve fluent generation in GraphSnapShot. As in the GraphSnapShot, the most important part of the way is to develop a great opportunity to achieve ...

\begin{table}[h]
\centering
\begin{tabular}{|c|c|c|c|}
\hline
\multirow{2}{*}{Method} & \multirow{2}{*}{Description} & \multicolumn{2}{c|}{Time (seconds)} \\ \cline{3-4} 
                      &                       & Average & Worst \\ \hline
Full Refresh (FR) + OTF Partial Fetch (PF) & Most Common & - & - \\ \hline
Partial Fetch (PF) + Partial Refresh (PR)  & Less Common & 0.23 & 0.82 \\ \hline
Partial Refresh (PR) + Partial Fetch (PF)  & Less Common & 0.54 & 0.54 \\ \hline
Partial Refresh (PR) + Full Fetch (FF)     & Less Common & 0.31 & 0.31 \\ \hline
\end{tabular}
\caption{Performance Comparison of Refresh and Fetch Methods}
\label{tab:performance}
\end{table}

Full Refresh (FR) + OTF Partial Fetch (PF) is the most commonly used method, leveraging full refresh alongside on-the-fly partial fetch, likely offering advantages in performance and efficiency, although no time data is provided. Partial Fetch (PF) + Partial Refresh (PR) exhibits a shorter average time of 0.23 seconds but a longer worst time of 0.82 seconds, indicating good performance in most cases but potential delays in certain scenarios due to its implementation of partial fetch and partial refresh. Partial Refresh (PR) + Partial Fetch (PF) has an average time of 0.54 seconds and a worst time of 0.54 seconds, showing more consistent performance across various scenarios, being closest to a graph structure query with each refresh. Partial Refresh (PR) + Full Fetch (FF) shows both an average and worst time of 0.31 seconds, similar to the second method in average time but excelling in worst-case scenarios, while also offering the best fluent generation due to its implementation of partial refresh and full fetch.




\subsection{Experimental Analysis of SSDReS Performance}

In our experiments, we explored the efficacy of the GraphSnapShot algorithm by testing the tradeoff between static and dynamic resampling. Static fetch (proportional to $fr$) focuses on quick access to graph topology information stored in memory. Dynamic resampling (proportional to \(rr\)), on the other hand, is a measurement for the memory swap, it addresses the real-time changes in the graph, frequently requiring access to disk-stored data and swap in the memory to update the in-memory topology.
% Give out the experimental analysis

% refresh rate is a measurement for the memory swap, where the $rr$ indicates for the the fract

Analyzing the outcomes of these experiments provides insights into the algorithm's performance:

\begin{itemize}
    \item \textbf{Accuracy and fetch rate}: 
    Our results showed a general increase in accuracy as fetch rate increased, which shows dynamic resampling has critical roles in enhancing model precision. A higher rate of dynamic resampling implies a greater reliance on the stable structure of the graph, aiding in capturing patterns in graph topology. A relative high dynamic resampling rate is beneficial for the model's training stability and generalizability.
    
    \item \textbf{Loss and fetch rate}: 
    Loss decreased with an increase in fetch rate, further validating the importance of dynamic resampling in improving model performance. Lower loss indicates reduced error in data fitting, suggesting that static resampling helps the algorithm to learn and predict the graph's structure more accurately. This could also imply that dynamic resampling offers a stable learning environment, potentially reducing the risk of overfitting.
    
    \item \textbf{Training Time and refresh rate}: 
    Our experiments indicated the existence of an optimal refresh rate value between 0 and 1, which minimizes training time, and with a little loss in acuracy. We call this point as "tradeoff" point between static and dynamic resampling. Over-dependence on dynamic resampling (low refresh rate) could increase the computational burden due to frequent updates required for rapidly changing graph structures, while excessive reliance on static resampling (high refresh rate) might cause the model to overly learn from limited portion of the graph structure in memory, deduce its ability to effectively learn from the entire graph structure. %miss recent changes in the graph structure.
    
\end{itemize}


The effectiveness of the GraphSnapShot algorithm lies in the way that it deploys disk-cache-memory architecture to store and update intermediate graph local structure (GraphSnapShot). By caching the K-V pairs of the reused graph structure, the graph machine learning is significantly accelerated. 

The GraphSnapShot excels in processing dynamic graph data and tasks that require exploration of graph structures, particularly for applications with complex and large-scale network structures.

\paragraph{Bridging the Gap Between Pure Dynamic Algorithms and Static Memory Storage with GraphSnapShot:} Dynamic graph algorithms, such as GraphSAGE, which require resampling the entire graph for each computation, incur significant overhead. This is primarily due to the need for constant, full-graph resampling to accommodate the ever-changing nature of dynamic graphs. GraphSnapShot addresses this issue by establishing a static snapshot at preprocessing phase and use dynamic processing to update partial snapshot at computation. This approach significantly reduces the computational burden by providing a stable, memory-stored snapshot (\textit{sG}) as a baseline.  GraphSnapShot ensures efficient computation and maintains the flexibility needed to handle dynamic changes in the graph.

\paragraph{Tradeoff Between Dynamic Sampling and Resampling:} In GraphSnapShot, the balance between dynamic sampling (\textit{DynamicSample}) and resampling (\textit{ReSample}) plays a pivotal role in maintaining an up-to-date representation of the graph. Dynamic sampling involves integrating new nodes from the disk into memory, capturing the latest updates and changes. Resampling, on the other hand, focuses on sampling and processing existing nodes from memory, which are then rotated back to disk storage. However, if \textit{DynamicSample} is too large, it is close to traditional sampling, resulting in prolonged disk retrieval times. Conversely, while resampling processes memory-stored nodes, an excessive \textit{ReSample} may overly rely on memory data, potentially leading to a decrease in accuracy. Striking this balance is essential: moderating dynamic sampling to prevent inefficiencies and ensuring resampling maintains graph accuracy without an undue dependence on memory. In short, this is a tradeoff between optimizing memory usage (quick accessing) and model accuracy.

\paragraph{Local Snapshot Swap Strategy:} The \textit{Add} and \textit{Remove} functions are designed to simulate the swap of nodes between memory and disk, reflecting the dynamic shifts between active and less active parts of the graph. This local snapshot swapping strategy is crucial for handling large-scale dynamic graphs, as it reduces the demand on memory and computational resources.

In conclusion, the design of our GraphSnapShot Process algorithm considers the complexity and variability of dynamic graph analysis. By combining static sampling with dynamic resampling, the algorithm effectively manages and analyzes graphs whose structures evolve over time, demonstrating robust performance and flexibility in handling large-scale network analyses.


==> content/gss_algs.tex <==
\section{Algorithmic Design}
As for the cache retrieval and refreshing methods, we develop three methods to simulate different strategies.

\subsection{FBL}
The first method is FBL, which is short for full batch load. FBL is the traditional method where most graph processing systems current are deployed. Those system does not caching any information and resample graph structure each time from disk to memory for computation.

\begin{figure}[H]
\centering
\includegraphics[width=1\linewidth]{figures/FBL.png}
\caption{FBL Cache Snapshot Strategy}
\end{figure}

% The second method is OTF, which is short for "on the fly", this method will partially update the cache while partially unchanged the cache information.

\subsection{OTF}
The "On The Fly" (OTF) method, updates portions of the cache dynamically while leaving other segments of the cache information unchanged. In detailed implementation of OTF, we design 4 different mode of it for real world application. They are (Full Fetch, Partial Fetch)x(Full Refresh, Partial Refresh).

In {*OTF-refresh*} mode, we implement a partial cache refresh strategy, which dynamically updates only a fraction of the cache based on a defined refresh rate.

\subsubsection{Algorithmic Design for OTF-refresh}
Let \( G = (V, E) \) denote a heterogeneous graph, where \( V \) and \( E \) represent the vertices and edges, respectively. The vertices are categorized by types, specified by \( \text{hete\_label} \).

\begin{itemize}
    \item \( \textbf{fanouts} = [f_1, f_2, \ldots, f_n] \): An array indicating the desired number of neighbors to sample at each depth level.
    \item \( \alpha \): A scaling factor for fanouts to determine the initial cache size for each depth.
    \item \( T \): The interval after which the cache is considered for partial refreshing.
    \item \( \gamma \): Refresh rate defining the fraction of the cache to update during each refresh cycle.
\end{itemize}

% \begin{algorithm}
% \caption{Neighbor Sampler with OTF Cache Refresh}
% \begin{algorithmic}[1]
% \Procedure{Initialize}{Graph $G$, Array fanouts, $\alpha$, $T$, $\gamma$, hete\_label}
%     \State Calculate cache sizes: $\text{cache\_size}[i] \gets f_i \times \alpha \text{ for each } i$
%     \State Initialize each cache layer by pre-sampling using calculated sizes
% \EndProcedure

% \Procedure{RefreshCache}{Layer ID, Cache Refresh Size}
%     \State Sample a portion of the current cache to retain
%     \State Sample new neighbors to replace the refreshed portion
%     \State Merge retained and new samples to update the cache
% \EndProcedure

% \Procedure{SampleBlocks}{Seed nodes $S$}
%     \If{current cycle modulo $T = 0$}
%         \For{each cache layer}
%             \State Refresh a portion of the cache based on $\gamma$
%         \EndFor
%     \EndIf
%     \For{each layer in reverse order}
%         \State Use the cache to sample blocks for seed nodes
%         \State Update seed nodes for the next layer
%     \EndFor
%     \State \Return Sampled blocks
% \EndProcedure
% \end{algorithmic}
% \end{algorithm}

\begin{algorithm}
\caption{Neighbor Sampling with OTF Cache Refresh}
\begin{algorithmic}[1]
\Procedure{Initialize}{$G, \{f_i\}, \alpha, T, \gamma, \ell$}
    \State $\text{cache\_size}_i \gets f_i \cdot \alpha, \; \forall i$
    \State Pre-sample and initialize $\text{cache}$ for each layer using $\{\text{cache\_size}_i\}$
\EndProcedure

\Procedure{RefreshCache}{$l, \gamma$}
    \State $n_\text{retain} \gets |\text{cache}[l]| \cdot (1 - \gamma)$
    \State $n_\text{new} \gets |\text{cache}[l]| \cdot \gamma$
    \State $N_\text{retain} \gets \text{SampleFromCache}(\text{cache}[l], n_\text{retain})$
    \State $N_\text{new} \gets \text{FetchFromDisk}(G, S, n_\text{new})$
    \State $\text{cache}[l] \gets N_\text{retain} \cup N_\text{new}$
\EndProcedure

\Procedure{SampleBlocks}{$S$}
    \If{$t \mod T = 0$}
        \For{$l = 1$ to $L$}
            \State \Call{RefreshCache}{$l, \gamma$}
        \EndFor
    \EndIf
    \For{$l = L$ to $1$}
        \State $N \gets \text{SampleFromCache}(S, f_l)$
        \State $S \gets N$
    \EndFor
    \State \Return $\text{blocks}$
\EndProcedure
\end{algorithmic}
\end{algorithm}

The OTF refresh strategy enhances the algorithm's responsiveness to changes in the graph's structure by updating a subset of the cache, thus balancing between computational efficiency and sampling accuracy. This approach is particularly beneficial in dynamic environments where frequent full cache refreshes are impractical.


\begin{figure}[H]
\centering
\includegraphics[width=1\linewidth]{figures/OTF.png}
\caption{OTF Cache Snapshot Strategy}
\end{figure}

In *OTF-fetch* mode, we design an algorithm that can maintaining up-to-date neighborhood information in dynamic graph environments. Traditional methods that rely solely on static pre-sampling can lead to stale data, affecting the model's performance. OTF-fetch mode introduces a fetching mechanism that balances between pre-sampled cache and real-time graph data, enhancing accuracy and efficiency.

\subsubsection{Algorithmic Design for OTF-fetch}
Let \( G = (V, E) \) be a heterogeneous graph, where \( V \) and \( E \) represent the vertices and edges, respectively. Each vertex belongs to a specific type, categorized under \( \text{hete\_label} \).

\begin{itemize}
    \item \( \textbf{fanouts} = [f_1, f_2, \ldots, f_n] \): An array indicating the number of neighbors to sample at each layer.
    \item \( \text{amp\_rate} \): Amplification rate that determines the size of the initial cache.
    \item \( T_{\text{fetch}} \): The period after which the cache is partially fetched to adjust the sample data dynamically.
    \item \( \text{fetch\_rate} \): Determines the fraction of the cache to be dynamically fetched alongside real-time data from the graph.
\end{itemize}

% \begin{algorithm}
% \caption{Neighbor Sampler with OTF Fetching Mechanism}
% \begin{algorithmic}[1]
% \Procedure{Initialize}{Graph $G$, Array fanouts, amp\_rate, T\_fetch, fetch\_rate, hete\_label}
%     \State Compute cache sizes: $\text{cache\_size}[i] \gets f_i \times \text{amp\_rate} \text{ for each } i$
%     \State Initialize each cache layer by pre-sampling using these sizes
% \EndProcedure

% \Procedure{OTF\_Fetch}{Layer ID, Seed Nodes, Fetch Size}
%     \State Compute the number of neighbors to fetch from the disk
%     \State Fetch required neighbors from the cache
%     \State Fetch additional neighbors directly from the graph
%     \State Merge both sets to form the updated sample
% \EndProcedure

% \Procedure{SampleBlocks}{Seed nodes $S$}
%     \For{each layer from last to first}
%         \State Determine the number of neighbors to fetch based on fetch\_rate
%         \If{current cycle modulo $T_{\text{fetch}} = 0$}
%             \State Call OTF\_Fetch to update sampled data
%         \Else
%             \State Sample directly from the pre-filled cache
%         \EndIf
%         \State Update seed nodes for the next layer
%     \EndFor
%     \State \Return Sampled blocks
% \EndProcedure
% \end{algorithmic}
% \end{algorithm}

\begin{algorithm}
\caption{Neighbor Sampler with OTF Fetching}
\begin{algorithmic}[1]
\Procedure{Initialize}{$G, \{f_i\}, \alpha, T_\text{fetch}, \beta, \ell$}
    \State $\text{cache\_size}_i \gets f_i \cdot \alpha, \; \forall i$
    \State Pre-sample caches with size $\text{cache\_size}_i$
\EndProcedure

\Procedure{OTF\_Fetch}{$l, S, n_\text{fetch}$}
    \State $n_\text{disk} \gets n_\text{fetch} - |\text{cache}|$
    \State $\text{neighbors} \gets \text{cache} \cup \text{FetchFromDisk}(G, S, n_\text{disk})$
    \State \Return $\text{neighbors}$
\EndProcedure

\Procedure{SampleBlocks}{$S$}
    \For{$l = L$ to $1$}
        \State $n_\text{fetch} \gets f_l \cdot \beta$
        \If{$t \mod T_\text{fetch} = 0$}
            \State $N \gets \text{OTF\_Fetch}(l, S, n_\text{fetch})$
        \Else
            \State $N \gets \text{SampleFromCache}(S, f_l)$
        \EndIf
        \State $S \gets N$
    \EndFor
    \State \Return $\text{blocks}$
\EndProcedure
\end{algorithmic}
\end{algorithm}

The OTF fetching strategy introduces a significant enhancement to graph sampling by allowing dynamic data retrieval, which integrates cached and real-time data. This mechanism ensures that the graph samples are both current and computationally efficient to retrieve, catering particularly well to environments where the graph's structure may change frequently. Moreover, this approach reduces the overhead associated with frequent full cache refreshes, thereby optimizing both memory usage and processing time.

\subsection{Algorithmic Design for OTF-partial fetch \& partial refresh}

Let \( G = (V, E) \) represent a heterogeneous graph where \( V \) and \( E \) denote the sets of vertices and edges, respectively, with vertices categorized by types specified by \( \text{hete\_label} \).

\begin{itemize}
    \item \( \textbf{fanouts} = [f_1, f_2, \ldots, f_n] \): Specifies the number of neighbors to sample at each depth.
    \item \( \text{amp\_rate} \): Amplification rate determining the initial cache size for each layer.
    \item \( T \): Period after which the cache is refreshed.
    \item \( \text{refresh\_rate} \): Proportion of the cache to be refreshed dynamically during each cycle.
\end{itemize}

% \begin{algorithm}
% \caption{Neighbor Sampling with OTF Partial Cache Fetch and Refresh}
% \begin{algorithmic}[1]
% \Procedure{Initialize}{Graph $G$, fanouts, amp\_rate, refresh\_rate, hete\_label}
%     \State Compute cache sizes using amp\_rate and fanouts.
%     \State Initialize cache for each layer.
% \EndProcedure

% \Procedure{OTF\_rf\_cache}{layer\_id, cached\_graph, seed\_nodes, refresh\_rate, fanout}
%     \State Calculate portions of the cache to refresh and fetch.
%     \State Fetch new data for specified portions while maintaining other data unchanged.
%     \State Update the cache dynamically to reflect recent changes.
% \EndProcedure

% \Procedure{SampleBlocks}{Graph $G$, seed\_nodes}
%     \For{each layer in cache}
%         \If{refresh required}
%             \State Call OTF\_rf\_cache to refresh and fetch data.
%         \EndIf
%         \State Use updated cache to sample blocks for seed nodes.
%         \State Update seed nodes for the next layer.
%     \EndFor
%     \State \Return Sampled blocks and updated seed nodes.
% \EndProcedure
% \end{algorithmic}
% \end{algorithm}

\begin{algorithm}
\caption{Neighbor Sampling with OTF Partial Cache Refresh}
\begin{algorithmic}[1]
\Procedure{Initialize}{$G, \{f_i\}, \alpha, \rho, \ell$}
    \State $\text{cache\_size}_i \gets f_i \cdot \alpha, \; \forall i$
    \State Pre-sample and initialize caches for each layer
\EndProcedure

\Procedure{OTF\_rf\_cache}{$l, \text{cache}, S, \rho, f_l$}
    \State $n_\text{refresh} \gets f_l \cdot \rho$
    \State $N_\text{new} \gets \text{FetchFromDisk}(G, S, n_\text{refresh})$
    \State $\text{cache}[l] \gets (\text{cache}[l] - \text{Stale}) \cup N_\text{new}$
    \State \Return $\text{cache}[l]$
\EndProcedure

\Procedure{SampleBlocks}{$G, S$}
    \For{$l = L$ to $1$}
        \If{$t \mod T_\text{refresh} = 0$}
            \State $\text{cache}[l] \gets \text{OTF\_rf\_cache}(l, \text{cache}[l], S, \rho, f_l)$
        \EndIf
        \State $N \gets \text{SampleFromCache}(S, f_l)$
        \State $S \gets N$
    \EndFor
    \State \Return $\text{blocks}$
\EndProcedure
\end{algorithmic}
\end{algorithm}

The OTF partial fetch and refresh strategy significantly enhances the responsiveness and accuracy of graph sampling in dynamic environments. By selectively updating the cache, the algorithm reduces computational overhead while maintaining high data freshness, crucial for downstream applications like machine learning where timely and accurate data is vital.

\subsection{OTF partial refresh \& full fetch}

OTF partial refresh \& full fetch is a mechanism for both partial cache refresh and full fetch. This methodology optimizes the sampling process by dynamically adjusting cache content to reflect the latest graph state, thus balancing computational efficiency with data freshness. 

Efficient graph sampling is pivotal in applications involving dynamic graphs, especially in scenarios where graph structures evolve over time. Traditional static caching methods often lead to outdated data, adversely affecting the performance of graph-based algorithms. Our approach, through dynamic cache management, ensures timely updates of the sampled data, significantly enhancing the relevance of the data used in downstream processes.


Let \( G = (V, E) \) denote a heterogeneous graph where \( V \) and \( E \) represent vertices and edges, respectively, categorized by \( \text{hete\_label} \).

\begin{itemize}
    \item \( \textbf{fanouts} = [f_1, f_2, \ldots, f_n] \): An array specifying the number of neighbors to sample at each depth.
    \item \( \text{amp\_rate} \): Amplification rate that determines the initial size of the cache for each depth.
    \item \( T \): Period after which the cache undergoes a refresh operation.
    \item \( \text{refresh\_rate} \): Proportion of the cache that is refreshed in each cycle.
\end{itemize}

% \begin{algorithm}
% \caption{Neighbor Sampling with OTF Partial Cache Refresh and Full Fetch}
% \begin{algorithmic}[1]
% \Procedure{Initialize}{Graph $G$, fanouts, amp\_rate, refresh\_rate, hete\_label}
%     \State Compute cache sizes using amp\_rate and fanouts.
%     \State Initialize cache for each layer.
% \EndProcedure

% \Procedure{OTF\_refresh\_cache}{layer\_id, cached\_graph, seed\_nodes, refresh\_rate}
%     \State Calculate the proportion of the cache to refresh.
%     \State Fetch new data for the refreshed portion while retaining other data unchanged.
%     \State Update the cache dynamically to incorporate recent graph changes.
% \EndProcedure

% \Procedure{SampleBlocks}{Graph $G$, seed\_nodes}
%     \For{each layer in cache}
%         \If{refresh required}
%             \State Call OTF\_refresh\_cache to refresh the data.
%         \EndIf
%         \State Fully fetch from the updated cache to sample blocks for seed nodes.
%         \State Update seed nodes for the next layer.
%     \EndFor
%     \State \Return Sampled blocks and updated seed nodes.
% \EndProcedure
% \end{algorithmic}
% \end{algorithm}

\begin{algorithm}
\caption{Neighbor Sampling with OTF Partial Cache Refresh and Full Fetch}
\begin{algorithmic}[1]
\Procedure{Initialize}{$G, \{f_i\}, \alpha, \rho, \ell$}
    \State $\text{cache\_size}_i \gets f_i \cdot \alpha, \; \forall i$
    \State Pre-sample and initialize caches for each layer
\EndProcedure

\Procedure{OTF\_refresh\_cache}{$l, \text{cache}, S, \rho$}
    \State $n_\text{refresh} \gets |\text{cache}[l]| \cdot \rho$
    \State $N_\text{new} \gets \text{FetchFromDisk}(G, S, n_\text{refresh})$
    \State $\text{cache}[l] \gets (\text{cache}[l] - \text{Stale}) \cup N_\text{new}$
    \State \Return $\text{cache}[l]$
\EndProcedure

\Procedure{SampleBlocks}{$G, S$}
    \For{$l = L$ to $1$}
        \If{$t \mod T_\text{refresh} = 0$}
            \State $\text{cache}[l] \gets \text{OTF\_refresh\_cache}(l, \text{cache}[l], S, \rho)$
        \EndIf
        \State $N \gets \text{SampleFromCache}(S, f_l)$
        \State $S \gets N$
    \EndFor
    \State \Return $\text{blocks}$
\EndProcedure
\end{algorithmic}
\end{algorithm}



\subsection{FCR}
The third method is FCR, which is short for "fully cache refreshing" in a batch. For FCR, in each batch, the the structure information are sampled from cache for computation, and between each batch, the cache is fully refreshed.

The Fully Cache Refresh (FCR) strategy effectively scales the depth and breadth of pre-sampled neighborhoods stored in the cache. This mechanism reduces the need for frequent neighborhood sampling from the graph, thereby lowering computational overhead and enhancing performance, especially in dynamic and large-scale heterogeneous graph environments. The periodic refresh rate $T$ ensures the cache remains up-to-date and reflects recent changes in the graph structure.

Let \( G = (V, E) \) be a heterogeneous graph where \( V \) and \( E \) represent vertices and edges respectively. The vertices may belong to different types, specified by \( \text{hete\_label} \).

\begin{itemize}
    \item \( \textbf{fanouts} = [f_1, f_2, \ldots, f_n] \): An array indicating the number of neighbors to sample at each depth of the sampling process.
    \item \( \alpha \): Fractional caching rate, controlling the scaling of \( \textbf{fanouts} \) for pre-sampling.
    \item \( T \): The interval after which the cache is refreshed to incorporate recent graph changes.
\end{itemize}

\begin{figure}[H]
\centering
\includegraphics[width=0.7\linewidth]{figures/FCR.png}
\caption{FCR Cache Snapshot Strategy}
\end{figure}

% ** FCR -pseduo code (how to with comparison to dgl FBL implementation)


% During the preprocessing phase, a static graph snapshot is sampled and stored to the memory from disk. In the computation phase, the graph snapshot for computation are resampled partillay from memory and partillay from disk, while a dynamic small snapshot is sampled from disk and used for swap into the memory to exchange the memory sampled one.

% GraphSnapShot combines advantanges of static and dynamic processing, where a static graph snapshot is stored at preprocessing phase, and the snapshot is capable of retrival and updating in the computation phase. was conceived to adeptly handle the complexities inherent in dynamic graph data, particularly in scenarios where the structure of the graph evolves over time. This algorithm is more than just a static data processing tool; it is a dynamic system capable of adapting to and updating the graph's structure in real time. 

% \paragraph{Addressing Dynamic Graph Challenges with Static Sampling Foundation:} The main challenge with dynamic graph data is its non-static, evolving nature. To effectively manage this dynamism, our GraphSnapShot algorithm initially employs a static sampling method to create a baseline snapshot (\textit{sG}), representing the initial state of the graph. This static snapshot provides a stable reference point, enabling comparison and quantification of changes in the graph’s structure.

% ** The shared cache mode.

% ** OTF extended implementation: Partial Refresh and Partial fetch.

% ** OTF - psuedo code

% \subsubsection{FCR Design}

Traditional methods often suffer from high computational costs due to repetitive neighborhood sampling. Our approach mitigates these issues by integrating a Fully Cache Refresh, which dictates the extent of neighborhood pre-sampling and cache utilization.

The Fully Cache Refresh approach, while ensuring the freshness of the sampled data, can be computationally intensive compared to partial or incremental refresh strategies, as it involves re-sampling large portions of the graph frequently. Therefore, it's crucial to carefully configure the refresh period T to balance performance with computational overhead, particularly in very large or rapidly-changing graphs.

This approach is ideal for scenarios where the accuracy and timeliness of the graph data are critical, such as in real-time monitoring systems or dynamic social networks where relationships and attributes may frequently change. By refreshing the entire cache periodically, the FCR method ensures that the sampling process remains robust and relevant to the current graph structure, thus supporting high-quality graph-based analyses and applications.

% \begin{algorithm}[H]
% \caption{NeighborSampler with Fully Cache Refresh}
% \begin{algorithmic}[1]
% \Procedure{Initialize}{Graph $G$, Array fanouts, $\alpha$, $T$, hete\_label}
%     \State $\text{amplified\_fanouts} \gets [f \times \alpha \text{ for } f \text{ in fanouts}]$
%     \State Initialize cache to empty
%     \State Pre-fill cache using $\text{amplified\_fanouts}$
% \EndProcedure

% \Procedure{CacheRefresh}{}
%     \State Clear cache
%     \State Re-sample neighborhoods using $\text{amplified\_fanouts}$
% \EndProcedure

% \Procedure{SampleBlocks}{Seed nodes $S$}
%     \If{current cycle modulo $T = 0$}
%         \State \Call{CacheRefresh}{}
%     \EndIf
%     \For{each level $k$ from $n$ down to 1}
%         \State Sample using cached neighborhoods
%         \State Update seed nodes for next level
%     \EndFor
%     \State \Return Sampled blocks
% \EndProcedure
% \end{algorithmic}
% \end{algorithm}

\begin{algorithm}
\caption{Neighbor Sampling with Fully Cache Refresh}
\begin{algorithmic}[1]
\Procedure{Initialize}{$G, \{f_i\}, \alpha, T, \ell$}
    \State $\text{amplified\_fanouts}_i \gets f_i \cdot \alpha, \; \forall i$
    \State $\text{cache} \gets \emptyset$
    \State Pre-sample and fill $\text{cache}$ using $\{\text{amplified\_fanouts}_i\}$
\EndProcedure

\Procedure{CacheRefresh}{}
    \State $\text{cache} \gets \emptyset$
    \State Re-sample neighborhoods into $\text{cache}$ using $\{\text{amplified\_fanouts}_i\}$
\EndProcedure

\Procedure{SampleBlocks}{$S$}
    \If{$t \mod T = 0$}
        \State \Call{CacheRefresh}{}
    \EndIf
    \For{$k = n$ to $1$}
        \State $N \gets \text{SampleFromCache}(S, f_k)$
        \State $S \gets N$
    \EndFor
    \State \Return $\text{blocks}$
\EndProcedure
\end{algorithmic}
\end{algorithm}

\subsection{Shared Cache Design}
Graph sampling is often computationally intensive, especially when dealing with large-scale heterogeneous graphs. The shared cache design aims to mitigate these challenges by maintaining a cache of pre-sampled neighborhoods, thus facilitating rapid access and reducing the frequency of expensive graph traversal operations.

Let \( G = (V, E) \) denote a heterogeneous graph where \( V \) and \( E \) represent the sets of vertices and edges, respectively. \( \text{fanouts} \) defines the number of neighbors to sample at each depth of sampling, and \( \alpha \) represents the scaling factor for cache size determination.

\begin{itemize}
    \item \( \text{fanouts} = [f_1, f_2, \ldots, f_n] \): Specifies the number of neighbors to sample at each layer.
    \item \( \alpha \): Amplification factor applied to each fanout to determine the initial cache size.
    \item \( T \): Period after which the cache is refreshed to ensure it remains representative of the graph's evolving structure.
\end{itemize}

\begin{algorithm}
\caption{Initialization and Refresh of Shared Cache}
\begin{algorithmic}[1]
\Procedure{Initialize}{Graph $G$, fanouts, alpha}
    \State $\text{sc\_size} \gets \max(fanouts) \times \alpha$ \Comment{Compute cache size}
    \State Pre-sample and populate cache using $G$, fanouts, and $\text{sc\_size}$
\EndProcedure

\Procedure{CacheRefresh}{}
    \If{current cycle modulo $T = 0$}
        \State Pre-sample neighborhoods to refresh the cache
    \EndIf
\EndProcedure
\end{algorithmic}
\end{algorithm}

The shared cache design effectively reduces the computational overhead associated with frequent and intensive graph sampling operations. By leveraging an amplified fanout strategy, the cache maintains a ready pool of neighborhood data that can be rapidly accessed during the sampling process, significantly enhancing performance and efficiency. The periodic refresh mechanism ensures the cache's data remains current, accommodating changes in the graph's topology over time.

==> content/gss_algs_simp.tex <==
\section{Algorithmic Design}
As for the cache retrieval and refreshing methods, we develop three methods to simulate different strategies.

\subsection{FBL}
The first method is FBL, which is short for full batch load. FBL is the traditional method where most graph processing systems current are deployed. Those system does not caching any information and resample graph structure each time from disk to memory for computation.

% \begin{figure}[H]
% \centering
% \includegraphics[width=1\linewidth]{figures/FBL.png}
% \caption{FBL Cache Snapshot Strategy}
% \end{figure}

% The second method is OTF, which is short for "on the fly", this method will partially update the cache while partially unchanged the cache information.

\subsection{OTF}
The "On The Fly" (OTF) method, updates portions of the cache dynamically while leaving other segments of the cache information unchanged. In detailed implementation of OTF, we design 4 different mode of it for real world application. They are (Full Fetch, Partial Fetch)x(Full Refresh, Partial Refresh).

In {*OTF-refresh*} mode, we implement a partial cache refresh strategy, which dynamically updates only a fraction of the cache based on a defined refresh rate.

\subsubsection{Algorithmic Design for OTF-refresh}
Let \( G = (V, E) \) denote a heterogeneous graph, where \( V \) and \( E \) represent the vertices and edges, respectively. The vertices are categorized by types, specified by \( \text{hete\_label} \).

\begin{itemize}
    \item \( \textbf{fanouts} = [f_1, f_2, \ldots, f_n] \): An array indicating the desired number of neighbors to sample at each depth level.
    \item \( \alpha \): A scaling factor for fanouts to determine the initial cache size for each depth.
    \item \( T \): The interval after which the cache is considered for partial refreshing.
    \item \( \gamma \): Refresh rate defining the fraction of the cache to update during each refresh cycle.
\end{itemize}

\begin{algorithm}
\caption{Neighbor Sampling with OTF Cache Refresh}
\begin{algorithmic}[1]
\Procedure{Initialize}{$G, \{f_i\}, \alpha, T, \gamma, \ell$}
    \State $\text{cache\_size}_i \gets f_i \cdot \alpha, \; \forall i$
    \State Pre-sample and initialize $\text{cache}$ for each layer using $\{\text{cache\_size}_i\}$
\EndProcedure

\Procedure{RefreshCache}{$l, \gamma$}
    \State $n_\text{retain} \gets |\text{cache}[l]| \cdot (1 - \gamma)$
    \State $n_\text{new} \gets |\text{cache}[l]| \cdot \gamma$
    \State $N_\text{retain} \gets \text{SampleFromCache}(\text{cache}[l], n_\text{retain})$
    \State $N_\text{new} \gets \text{FetchFromDisk}(G, S, n_\text{new})$
    \State $\text{cache}[l] \gets N_\text{retain} \cup N_\text{new}$
\EndProcedure

\Procedure{SampleBlocks}{$S$}
    \If{$t \mod T = 0$}
        \For{$l = 1$ to $L$}
            \State \Call{RefreshCache}{$l, \gamma$}
        \EndFor
    \EndIf
    \For{$l = L$ to $1$}
        \State $N \gets \text{SampleFromCache}(S, f_l)$
        \State $S \gets N$
    \EndFor
    \State \Return $\text{blocks}$
\EndProcedure
\end{algorithmic}
\end{algorithm}

The OTF refresh strategy enhances the algorithm's responsiveness to changes in the graph's structure by updating a subset of the cache, thus balancing between computational efficiency and sampling accuracy. This approach is particularly beneficial in dynamic environments where frequent full cache refreshes are impractical.


% \begin{figure}[H]
% \centering
% \includegraphics[width=1\linewidth]{figures/OTF.png}
% \caption{OTF Cache Snapshot Strategy}
% \end{figure}

In *OTF-fetch* mode, we design an algorithm that can maintaining up-to-date neighborhood information in dynamic graph environments. Traditional methods that rely solely on static pre-sampling can lead to stale data, affecting the model's performance. OTF-fetch mode introduces a fetching mechanism that balances between pre-sampled cache and real-time graph data, enhancing accuracy and efficiency.

\subsubsection{Algorithmic Design for OTF-fetch}
Let \( G = (V, E) \) be a heterogeneous graph, where \( V \) and \( E \) represent the vertices and edges, respectively. Each vertex belongs to a specific type, categorized under \( \text{hete\_label} \).

\begin{itemize}
    \item \( \textbf{fanouts} = [f_1, f_2, \ldots, f_n] \): An array indicating the number of neighbors to sample at each layer.
    \item \( \text{amp\_rate} \): Amplification rate that determines the size of the initial cache.
    \item \( T_{\text{fetch}} \): The period after which the cache is partially fetched to adjust the sample data dynamically.
    \item \( \text{fetch\_rate} \): Determines the fraction of the cache to be dynamically fetched alongside real-time data from the graph.
\end{itemize}

\begin{algorithm}
\caption{Neighbor Sampler with OTF Fetching}
\begin{algorithmic}[1]
\Procedure{Initialize}{$G, \{f_i\}, \alpha, T_\text{fetch}, \beta, \ell$}
    \State $\text{cache\_size}_i \gets f_i \cdot \alpha, \; \forall i$
    \State Pre-sample caches with size $\text{cache\_size}_i$
\EndProcedure

\Procedure{OTF\_Fetch}{$l, S, n_\text{fetch}$}
    \State $n_\text{disk} \gets n_\text{fetch} - |\text{cache}|$
    \State $\text{neighbors} \gets \text{cache} \cup \text{FetchFromDisk}(G, S, n_\text{disk})$
    \State \Return $\text{neighbors}$
\EndProcedure

\Procedure{SampleBlocks}{$S$}
    \For{$l = L$ to $1$}
        \State $n_\text{fetch} \gets f_l \cdot \beta$
        \If{$t \mod T_\text{fetch} = 0$}
            \State $N \gets \text{OTF\_Fetch}(l, S, n_\text{fetch})$
        \Else
            \State $N \gets \text{SampleFromCache}(S, f_l)$
        \EndIf
        \State $S \gets N$
    \EndFor
    \State \Return $\text{blocks}$
\EndProcedure
\end{algorithmic}
\end{algorithm}

The OTF fetching strategy introduces a significant enhancement to graph sampling by allowing dynamic data retrieval, which integrates cached and real-time data. This mechanism ensures that the graph samples are both current and computationally efficient to retrieve, catering particularly well to environments where the graph's structure may change frequently. Moreover, this approach reduces the overhead associated with frequent full cache refreshes, thereby optimizing both memory usage and processing time.

\subsection{Algorithmic Design for OTF-partial fetch \& partial refresh}

Let \( G = (V, E) \) represent a heterogeneous graph where \( V \) and \( E \) denote the sets of vertices and edges, respectively, with vertices categorized by types specified by \( \text{hete\_label} \).

\begin{itemize}
    \item \( \textbf{fanouts} = [f_1, f_2, \ldots, f_n] \): Specifies the number of neighbors to sample at each depth.
    \item \( \text{amp\_rate} \): Amplification rate determining the initial cache size for each layer.
    \item \( T \): Period after which the cache is refreshed.
    \item \( \text{refresh\_rate} \): Proportion of the cache to be refreshed dynamically during each cycle.
\end{itemize}

\begin{algorithm}
\caption{Neighbor Sampling with OTF Partial Cache Refresh}
\begin{algorithmic}[1]
\Procedure{Initialize}{$G, \{f_i\}, \alpha, \rho, \ell$}
    \State $\text{cache\_size}_i \gets f_i \cdot \alpha, \; \forall i$
    \State Pre-sample and initialize caches for each layer
\EndProcedure

\Procedure{OTF\_rf\_cache}{$l, \text{cache}, S, \rho, f_l$}
    \State $n_\text{refresh} \gets f_l \cdot \rho$
    \State $N_\text{new} \gets \text{FetchFromDisk}(G, S, n_\text{refresh})$
    \State $\text{cache}[l] \gets (\text{cache}[l] - \text{Stale}) \cup N_\text{new}$
    \State \Return $\text{cache}[l]$
\EndProcedure

\Procedure{SampleBlocks}{$G, S$}
    \For{$l = L$ to $1$}
        \If{$t \mod T_\text{refresh} = 0$}
            \State $\text{cache}[l] \gets \text{OTF\_rf\_cache}(l, \text{cache}[l], S, \rho, f_l)$
        \EndIf
        \State $N \gets \text{SampleFromCache}(S, f_l)$
        \State $S \gets N$
    \EndFor
    \State \Return $\text{blocks}$
\EndProcedure
\end{algorithmic}
\end{algorithm}

The OTF partial fetch and refresh strategy significantly enhances the responsiveness and accuracy of graph sampling in dynamic environments. By selectively updating the cache, the algorithm reduces computational overhead while maintaining high data freshness, crucial for downstream applications like machine learning where timely and accurate data is vital.

\subsection{OTF partial refresh \& full fetch}

OTF partial refresh \& full fetch is a mechanism for both partial cache refresh and full fetch. This methodology optimizes the sampling process by dynamically adjusting cache content to reflect the latest graph state, thus balancing computational efficiency with data freshness. 

Efficient graph sampling is pivotal in applications involving dynamic graphs, especially in scenarios where graph structures evolve over time. Traditional static caching methods often lead to outdated data, adversely affecting the performance of graph-based algorithms. Our approach, through dynamic cache management, ensures timely updates of the sampled data, significantly enhancing the relevance of the data used in downstream processes.


Let \( G = (V, E) \) denote a heterogeneous graph where \( V \) and \( E \) represent vertices and edges, respectively, categorized by \( \text{hete\_label} \).

\begin{itemize}
    \item \( \textbf{fanouts} = [f_1, f_2, \ldots, f_n] \): An array specifying the number of neighbors to sample at each depth.
    \item \( \text{amp\_rate} \): Amplification rate that determines the initial size of the cache for each depth.
    \item \( T \): Period after which the cache undergoes a refresh operation.
    \item \( \text{refresh\_rate} \): Proportion of the cache that is refreshed in each cycle.
\end{itemize}

\begin{algorithm}
\caption{Neighbor Sampling with OTF Partial Cache Refresh and Full Fetch}
\begin{algorithmic}[1]
\Procedure{Initialize}{$G, \{f_i\}, \alpha, \rho, \ell$}
    \State $\text{cache\_size}_i \gets f_i \cdot \alpha, \; \forall i$
    \State Pre-sample and initialize caches for each layer
\EndProcedure

\Procedure{OTF\_refresh\_cache}{$l, \text{cache}, S, \rho$}
    \State $n_\text{refresh} \gets |\text{cache}[l]| \cdot \rho$
    \State $N_\text{new} \gets \text{FetchFromDisk}(G, S, n_\text{refresh})$
    \State $\text{cache}[l] \gets (\text{cache}[l] - \text{Stale}) \cup N_\text{new}$
    \State \Return $\text{cache}[l]$
\EndProcedure

\Procedure{SampleBlocks}{$G, S$}
    \For{$l = L$ to $1$}
        \If{$t \mod T_\text{refresh} = 0$}
            \State $\text{cache}[l] \gets \text{OTF\_refresh\_cache}(l, \text{cache}[l], S, \rho)$
        \EndIf
        \State $N \gets \text{SampleFromCache}(S, f_l)$
        \State $S \gets N$
    \EndFor
    \State \Return $\text{blocks}$
\EndProcedure
\end{algorithmic}
\end{algorithm}



\subsection{FCR}
The third method is FCR, which is short for "fully cache refreshing" in a batch. For FCR, in each batch, the the structure information are sampled from cache for computation, and between each batch, the cache is fully refreshed.

The Fully Cache Refresh (FCR) strategy effectively scales the depth and breadth of pre-sampled neighborhoods stored in the cache. This mechanism reduces the need for frequent neighborhood sampling from the graph, thereby lowering computational overhead and enhancing performance, especially in dynamic and large-scale heterogeneous graph environments. The periodic refresh rate $T$ ensures the cache remains up-to-date and reflects recent changes in the graph structure.

Let \( G = (V, E) \) be a heterogeneous graph where \( V \) and \( E \) represent vertices and edges respectively. The vertices may belong to different types, specified by \( \text{hete\_label} \).

\begin{itemize}
    \item \( \textbf{fanouts} = [f_1, f_2, \ldots, f_n] \): An array indicating the number of neighbors to sample at each depth of the sampling process.
    \item \( \alpha \): Fractional caching rate, controlling the scaling of \( \textbf{fanouts} \) for pre-sampling.
    \item \( T \): The interval after which the cache is refreshed to incorporate recent graph changes.
\end{itemize}

% \begin{figure}[H]
% \centering
% \includegraphics[width=0.7\linewidth]{figures/FCR.png}
% \caption{FCR Cache Snapshot Strategy}
% \end{figure}

Traditional methods often suffer from high computational costs due to repetitive neighborhood sampling. Our approach mitigates these issues by integrating a Fully Cache Refresh, which dictates the extent of neighborhood pre-sampling and cache utilization.

The Fully Cache Refresh approach, while ensuring the freshness of the sampled data, can be computationally intensive compared to partial or incremental refresh strategies, as it involves re-sampling large portions of the graph frequently. Therefore, it's crucial to carefully configure the refresh period T to balance performance with computational overhead, particularly in very large or rapidly-changing graphs.

This approach is ideal for scenarios where the accuracy and timeliness of the graph data are critical, such as in real-time monitoring systems or dynamic social networks where relationships and attributes may frequently change. By refreshing the entire cache periodically, the FCR method ensures that the sampling process remains robust and relevant to the current graph structure, thus supporting high-quality graph-based analyses and applications.

\begin{algorithm}
\caption{Neighbor Sampling with Fully Cache Refresh}
\begin{algorithmic}[1]
\Procedure{Initialize}{$G, \{f_i\}, \alpha, T, \ell$}
    \State $\text{amplified\_fanouts}_i \gets f_i \cdot \alpha, \; \forall i$
    \State $\text{cache} \gets \emptyset$
    \State Pre-sample and fill $\text{cache}$ using $\{\text{amplified\_fanouts}_i\}$
\EndProcedure

\Procedure{CacheRefresh}{}
    \State $\text{cache} \gets \emptyset$
    \State Re-sample neighborhoods into $\text{cache}$ using $\{\text{amplified\_fanouts}_i\}$
\EndProcedure

\Procedure{SampleBlocks}{$S$}
    \If{$t \mod T = 0$}
        \State \Call{CacheRefresh}{}
    \EndIf
    \For{$k = n$ to $1$}
        \State $N \gets \text{SampleFromCache}(S, f_k)$
        \State $S \gets N$
    \EndFor
    \State \Return $\text{blocks}$
\EndProcedure
\end{algorithmic}
\end{algorithm}

\subsection{Shared Cache Design}
Graph sampling is often computationally intensive, especially when dealing with large-scale heterogeneous graphs. The shared cache design aims to mitigate these challenges by maintaining a cache of pre-sampled neighborhoods, thus facilitating rapid access and reducing the frequency of expensive graph traversal operations.

Let \( G = (V, E) \) denote a heterogeneous graph where \( V \) and \( E \) represent the sets of vertices and edges, respectively. \( \text{fanouts} \) defines the number of neighbors to sample at each depth of sampling, and \( \alpha \) represents the scaling factor for cache size determination.

\begin{itemize}
    \item \( \text{fanouts} = [f_1, f_2, \ldots, f_n] \): Specifies the number of neighbors to sample at each layer.
    \item \( \alpha \): Amplification factor applied to each fanout to determine the initial cache size.
    \item \( T \): Period after which the cache is refreshed to ensure it remains representative of the graph's evolving structure.
\end{itemize}

\begin{algorithm}
\caption{Initialization and Refresh of Shared Cache}
\begin{algorithmic}[1]
\Procedure{Initialize}{Graph $G$, fanouts, alpha}
    \State $\text{sc\_size} \gets \max(fanouts) \times \alpha$ \Comment{Compute cache size}
    \State Pre-sample and populate cache using $G$, fanouts, and $\text{sc\_size}$
\EndProcedure

\Procedure{CacheRefresh}{}
    \If{current cycle modulo $T = 0$}
        \State Pre-sample neighborhoods to refresh the cache
    \EndIf
\EndProcedure
\end{algorithmic}
\end{algorithm}

The shared cache design effectively reduces the computational overhead associated with frequent and intensive graph sampling operations. By leveraging an amplified fanout strategy, the cache maintains a ready pool of neighborhood data that can be rapidly accessed during the sampling process, significantly enhancing performance and efficiency. The periodic refresh mechanism ensures the cache's data remains current, accommodating changes in the graph's topology over time.

==> content/intro.tex <==
\section{Introduction}

In our recent research, we have developed a framework called GraphSnapShot, which has been proven an useful tool for graph learning acceleration. The core idea of GraphSnapShot is to capture and update the state of local graph structures dynamically, just like taking snapshots of graphs. 

GraphSnapShot is designed to efficiently capture, store and update the dynamic snapshots of graph data, enabling us to track patterns in the structure of graph networks. This technique is useful for most graph learning tasks that relies on topology analysis or networks are constantly evolving, such as social media analysis, biological networks, or any system where the relationships between entities change over time.

The key components of GraphSnapShot is the GraphSDSampler. GraphSDSampler can efficiently capture, update, retrieve and store graph snapshots of topology while doing computation at the same time, which makes graph learning computation significantly faster.

In experiments, GraphSnapShot shows efficiency. It can promote computation speed significantly compared to traditional NeighborhodSamplers implemented in dgl \cite{wang2019deep}, and it can reduce the GPU \& memory usage during training, with little loss of accuracy.
% K-hop Sampling Methods in local topology storage and retrival (in 2-hop, 3-hop and 4-hop domain), with little loss of accuracy. 
Experimental results show that the GraphSnapShot has potential to be a powerful tool for large graph training acceleration.

==> content/model_construction.tex <==
\section{Model Construction}

GraphSnapShot introduces caching masked graph structure for graph learning acceleration. The main process of GraphSnapShot involves two phases: preprocess sampling and dynamic resampling, both are methods for caching graph mask. 

Traditional graph learning methods struggle with extensive memory usage and slow computation. Node-wise sampling methods, including well-known ones like GraphSAGE \citep{hamilton2017inductive}, are not optimized for multi-hop scenarios due to the computational resources usage that grows exponentially with each additional hop— a phenomenon known as the "neighbor explosion." This makes them unsuitable for large-scale graphs where the capture of extended neighborhoods is crucial. Layer-wise sampling, such as in FastGCN\citep{chen2018fastgcn}, although designed to mitigate this explosion by sampling nodes per layer, often loses valuable connectivity information, leading to a sparse and inaccurate representation of the graph's multi-hop structure. Furthermore, subgraph sampling methods such as Cluster-GCN \citep{Chiang_2019} focus on localized computations and overlook vital inter-subgraph connections, failing to capture the broader topology necessary for a comprehensive multi-hop domain analysis.

GraphSnapShot's core idea is to achieve efficient cache management in graph learning, it is designed to maintain an up-to-date cache through the following strategies:

\begin{itemize}
    \item \textbf{Fully Cache Refresh (FCR):} Periodically refresh the whole cache to get a new representative of the graph local structure.

    \item \textbf{On-The-Fly (OTF):} Retreive the new representation of graph local structure in each computation, with partially retrieve from the previous graph local structure and partially retrieve from the disk.
    In detail the OTF can be identified as follows based on their fetch and refresh methods:
    \begin{itemize}
        \item \textbf{Partial Cache Refresh and Full Fetch}: Dynamically updates portions of the cache or retrieves all data from cache for computation as needed.
        \item \textbf{Partial Refresh with Partial Fetch}: OTF method in partially updating and partially retrieving data from both disk and cache, balancing cache up-to-date cache with computational efficiency.
        \item \textbf{Only Fetch Mode}: Fetch data for computation from cache by OTF mode with update existing cache periodically.
        \item \textbf{Only Refresh Mode}: Updates the existing cache by OTF mode.
    \end{itemize}

    \item \textbf{Shared Cache Mode:} Unlike traditional methods that cache individual nodes or edges, this mode involves caching significant portions of the graph that are frequently accessed by various processes. This strategy optimizes memory usage and ensures that the most frequently accessed data is readily available, enhancing the responsiveness and efficiency of graph machine learning tasks.
\end{itemize}

% Another method is for the shared cache mode for the local structure, as for the ...

% Give out the Pseudo-code for the Experiment.

% Give out the model figure.

==> content/motivation.tex <==
\section{Motivation} 

In machine learning, masks are powerful tools for reducing computation and enhancing model efficiency. In attention masks of long sequences, models selectively attend to relevant tokens within sequences, bypassing unnecessary computations and enabling more focused processing. Masks can also find utility in regularization techniques like dropout, where they aid in randomly deactivating units during training, thus preventing overfitting and promoting generalization. Additionally, in tasks such as instance segmentation in computer vision, masks efficiently delineate object boundaries, streamlining the computational load by restricting processing to specific regions of interest. Through these mechanisms, masks can reduce computational resources and contribute to the scalability of machine learning models. Notably, masked language modeling \citep{song2019mass, wettig2022should} and masked vision learning \citep{li2023scaling} showcase the significance of masks.



Although masks are widely used in NLP and computer vision, their applications in graph learning are limited. In this study, we propose GraphSnapShot, a novel method for cache-masked graph structure learning. The aim of GraphSnapShot is to reduce computational resources and accelerate the speed of graph machine learning at large scale.

% \subsection{Masked Language Modeling}

% \begin{figure}[H]
% \centering
% \includegraphics[width=0.4\linewidth]{figures/masked_language_modeling.png}
% \caption{Masked in Auto-Regressive Prediction in Language Modeling}
% \end{figure}


% \subsection{Masked Computer Vision}

% \begin{figure}[H]
%     \centering
%     \begin{subfigure}{.3\textwidth}
%         \centering
%         \includegraphics[width=\linewidth]{figures/pike.png}
%     \end{subfigure}%
%     \begin{subfigure}{.3\textwidth}
%         \centering
%         \includegraphics[width=\linewidth]{figures/masked_pike_1.png}
%     \end{subfigure}%
%     \begin{subfigure}{.3\textwidth}
%         \centering
%         \includegraphics[width=\linewidth]{figures/masked_pike_2.png}
%     \end{subfigure}
%     \caption{Mask Techinques in Comrputer Vision}
% \end{figure}

% \subsection{Masked Graph Machine Learning}

% \begin{figure}[H]
% \centering
% \includegraphics[width=0.7\linewidth]{figures/graph_mask.png}
% \caption{Mask in Graph Machine Learning}
% \end{figure}


==> content/overview.tex <==
\section{GraphSnapShot Overview}
\begin{figure}[H]
\centering
\includegraphics[width=1\linewidth]{figures/dense_proc.png}
\caption{Graph Processing Overview of GraphSnapShot}
\end{figure}

Our approach involves splitting a graph into two subgraphs based on the node degree threshold. Nodes with a degree higher than a specified threshold are categorized into a dense subgraph, while those with a degree below the threshold form a sparse subgraph. This division allows for the application of different sampling techniques to each subgraph, optimizing the computational resources and processing time.

For dense subgraphs, we utilize advanced sampling methods in GraphSnapShot such as FCR, OTF, FCR-SC, OTF-SC, etc, which are designed to efficiently manage the memory cache while maintaining the quality of the sampled neighborhood. These samplers dynamically adjust their sampling rates and cache refresh rates based on the learning phase and node centrality, ensuring efficient processing of dense regions.

For sparse subgraphs, we employ a Full Batch Load (FBL) approach, akin to DGL's NeighborSampler. This method is suitable for areas of the graph with lower degrees, where the computational overhead is inherently less, allowing for direct processing without the need for intricate sampling techniques.

We use the Deep Graph Library (DGL\citep{wang2019deep}) framework to implement new samplers in GraphSnapShot, leveraging its efficient handling of graph data structures and operations. Our implementation involves loading the graph, applying the graph splitting based on node degree, and then processing each subgraph with the respective sampling technique. We evaluated the performance of our new models on datasets in ogbn-benchmark\citep{hu2020open}. The results show that GraphSnapShot can significantly reduce training time and memory usage without compromising the quality of GNN training.


\paragraph{Bridging the Gap Between Pure Dynamic Algorithms and Static Memory Storage with GraphSnapShot:} Dynamic graph algorithms, such as GraphSAGE, which require resampling the entire graph for each computation, incur significant overhead. This is primarily due to the need for constant, full-graph resampling to accommodate the ever-changing nature of dynamic graphs. GraphSnapShot addresses this issue by establishing a static snapshot at preprocessing phase and use dynamic processing to update partial snapshot at computation. This approach significantly reduces the computational burden by providing a stable, memory-stored snapshot (\textit{sG}) as a baseline.  GraphSnapShot ensures efficient computation and maintains the flexibility needed to handle dynamic changes in the graph.

%This baseline snapshot, representing the initial state of the graph, offers rapid access and retrieval, creating a stark contrast with the high overhead of pure dynamic algorithms. The static snapshot serves as a reliable reference point, against which changes in the graph's structure can be effectively measured and analyzed.


% \paragraph{Tradeoff Dynamic Sampling and Resampling:} The dynamic sampling (\textit{DynamicSample}) and resampling (\textit{ReSample}) steps in the algorithm are key to updating the graph’s current state in real-time. By dynamically sampling and update new nodes from the disk to memory and resampling existing nodes from memory for computation and swap them into disk, the algorithm captures the immediate changes in the graph. %This design allows the algorithm to respond effectively to dynamic changes while maintaining a static baseline. The reason for this dynamic sampling approach is to ensure that the GraphSnapShot remains efficient and accurate, especially when handling large-scale and complex networks.

\paragraph{Tradeoff Between Dynamic Sampling and Resampling:} In GraphSnapShot, the balance between dynamic sampling (\textit{DynamicSample}) and resampling (\textit{ReSample}) plays a pivotal role in maintaining an up-to-date representation of the graph. Dynamic sampling involves integrating new nodes from the disk into memory, capturing the latest updates and changes. Resampling, on the other hand, focuses on sampling and processing existing nodes from memory, which are then rotated back to disk storage. However, if \textit{DynamicSample} is too large, it is close to traditional sampling, resulting in prolonged disk retrieval times. Conversely, while resampling processes memory-stored nodes, an excessive \textit{ReSample} may overly rely on memory data, potentially leading to a decrease in accuracy. Striking this balance is essential: moderating dynamic sampling to prevent inefficiencies and ensuring resampling maintains graph accuracy without an undue dependence on memory. In short, this is a tradeoff between optimizing memory usage (quick accessing) and model accuracy.

% This equilibrium ensures that GraphSnapShot remains both efficient and accurate, adeptly managing dynamic graph data while optimizing memory use.

%This interplay ensures that the graph's current state is accurately reflected in real-time. The dynamic sampling keeps the snapshot current with new information, while resampling manages memory efficiently by only retaining the most relevant data for active computation. This approach successfully negotiates the need for current, comprehensive graph data with the constraints of memory capacity, offering an optimized solution for dynamic graph management.

\paragraph{Local Snapshot Swap Strategy:} The \textit{Add} and \textit{Remove} functions are designed to simulate the swap of nodes between memory and disk, reflecting the dynamic shifts between active and less active parts of the graph. This local snapshot swapping strategy is crucial for handling large-scale dynamic graphs, as it reduces the demand on memory and computational resources.

% \paragraph{Flexibility in Computation and Termination Conditions:} The computation step (\textit{Compute}) within the \textit{Process} function is designed to be flexible and customizable according to different application needs. The setting of termination conditions reflects the algorithm's adaptability and flexibility in practical applications, ensuring timely conclusion and delivery of the final results.

In conclusion, the design of our GraphSnapShot Process algorithm considers the complexity and variability of dynamic graph analysis. By combining static sampling with dynamic resampling, the algorithm effectively manages and analyzes graphs whose structures evolve over time, demonstrating robust performance and flexibility in handling large-scale network analyses.

\paragraph{Dense \& Sparse Graphs Processing:} Our approach shows significant improvements in computational efficiency compared to traditional methods. The dual sampling strategy for dense and sparse graphs allows for targeted resource allocation, effectively handling dense and sparse regions within the graph. By using FBL, sparse graph processing can avoid resampled on same node set; by using GraphSnapShot, dense graph processing can have smaller cache size and quicker processing time. This results in faster training times without compromising the accuracy of the GNN models. Belows are figures to visulize the sample efficiency for Dense \& Sparse Processing.

\begin{algorithm}
\caption{Calculate Total Degree}
\begin{algorithmic}[1]
\State \textbf{Input:} Heterogeneous graph $G$, node type $t$
\State \textbf{Output:} Array $\text{total\_degrees}$

\State $\text{total\_degrees} \gets$ array of zeros, size equal to $|G_t|$ (number of nodes of type $t$ in $G$)
\For{each $(s, r, d)$ in $G.\text{edge\_types}$}
    \If{$d = t$}
        \State $\text{total\_degrees} \gets \text{total\_degrees} + G.\text{in\_degrees}((s, r, d))$
    \EndIf
    \If{$s = t$}
        \State $\text{total\_degrees} \gets \text{total\_degrees} + G.\text{out\_degrees}((s, r, d))$
    \EndIf
\EndFor
\State \Return $\text{total\_degrees}$
\end{algorithmic}
\end{algorithm}

\begin{algorithm}
\caption{Split Graph by Degree}
\begin{algorithmic}[1]
\State \textbf{Input:} Heterogeneous graph $G$, node type $t$, degree threshold $\theta$
\State \textbf{Output:} Subgraphs $G_{\text{high}}, G_{\text{low}}$

\State $\text{total\_degrees} \gets \Call{Calculate\_Total\_Degree}{G, t}$
\State $\text{high\_nodes} \gets$ indices where $\text{total\_degrees} > \theta$
\State $\text{low\_nodes} \gets$ indices where $\text{total\_degrees} \leq \theta$
\State $G_{\text{high}} \gets G.\text{subgraph}(\text{high\_nodes})$
\State $G_{\text{low}} \gets G.\text{subgraph}(\text{low\_nodes})$
\State \Return $G_{\text{high}}, G_{\text{low}}$
\end{algorithmic}
\end{algorithm}

\begin{figure}[H]
\centering
\includegraphics[width=1\linewidth]{figures/sample_efficiency_homo_arxiv.png}
\caption{Dense and Sparse Processing for ogbn-arixv}
\end{figure}

\begin{figure}[H]
\centering
\includegraphics[width=1\linewidth]{figures/sample_efficiency_homo_products.png}
\caption{Dense and Sparse Processing for ogbn-products}
\end{figure}


\begin{figure}[H]
\centering
\includegraphics[width=1\linewidth]{figures/sample_efficiency_hete_mag.png}
\caption{Dense and Sparse Processing for ogbn-mag}
\end{figure}

